Classifier-Free Guidance inside the Attraction Basin May Cause Memorization

Diffusion models are prone to exactly reproduce images from the training data. This exact reproduction of the training data is concerning as it can lead to copyright infringement and/or leakage of privacy-sensitive information. In this paper, we present a novel perspective on the memorization phenomenon and propose a simple yet effective approach to mitigate it. We argue that memorization occurs because of an attraction basin in the denoising process which steers the diffusion trajectory towards a memorized image. However, this can be mitigated by guiding the diffusion trajectory away from the attraction basin by not applying classifier-free guidance until an ideal transition point occurs from which classifier-free guidance is applied. This leads to the generation of non-memorized images that are high in image quality and well-aligned with the conditioning mechanism. To further improve on this, we present a new guidance technique, opposite guidance, that escapes the attraction basin sooner in the denoising process. We demonstrate the existence of attraction basins in various scenarios in which memorization occurs, and we show that our proposed approach successfully mitigates memorization.

==> definitions/definition1_backup.tex <==
Let $X$ denotes the entire state space of the diffusion trajectory at each time step and \( X_t \in X \) be the state space at time \( t \). Let \( \varphi_t: X \to X \) denote the reverse diffusion process with CFG such that \( \varphi_t(x) \) represents the state of the trajectory at time \( t \), starting from a state \( x \in X \).

Let \( A \subseteq X \) be an attractor for the system, meaning that A is the state toward which the diffusion trajectories denoised with CFG tend to converge at $t=0$, despite the initial noise. More formally, A is an attractor if there exists a region \( B(A, \epsilon) \) such that the probability of a trajectory starting from a point in \( B(A, \epsilon) \) and converging to A over time is high irrespective of the initial state. We have, 
\[
B(A, \epsilon) = \left\{ x \in X \mid \mathbb{P}(\lim_{t \to 0} \varphi_t(x) \in A) = 1-\epsilon \right\}.
\]
This set represents all points in the state space whose trajectories, when evolved over time using CFG, will end up at the attractor \( A \).


==> definitions/definition2_backup.tex <==
Let $X$ denotes the entire state space of the diffusion trajectory at each time step and \( X_t \in X \) be the state space at time \( t \). Let \( \varphi_t: X \to X \) denote the reverse diffusion process with CFG such that \( \varphi_t(x) \) represents the state of the trajectory at time \( t \), starting from a state \( x \in X \). Let \( A \subseteq X \) be an attractor for the system and \( B(A, \epsilon) \) be the attraction basin. We define the transition point as \( (x_{\tau}, \tau) \) for \( x_{\tau} \in X_{\tau} \) and $\tau>0$ at which applying CFG will not lead to the attractor A. More formally, 
% \[
%      \mathbb{P}( \lim_{t \to 0} \varphi_t(x_{\tau}) \in A) = 0  \quad \text{and} \quad  \mathbb{P}( \lim_{t \to 0} \varphi_t(x_{\tau-1}) \in A) = 1. 
% \]
\[
     \mathbb{P}( \lim_{t \to 0} \varphi_t(x_{\tau+1}) \in A) = 1 - \epsilon; \quad \mathbb{P}( \lim_{t \to 0} \varphi_t(x_{\tau}) \in A) = \epsilon. 
\]
